Conservative Galerkin methods for dispersive Hamiltonian problems

An energy conservative discontinuous Galerkin scheme for a generalised third order KdV type equation is designed. Based on the conservation principle, we propose techniques that allow for the derivation of optimal a priori bounds for the linear KdV equation and a posteriori bounds for the linear and modified KdV equation. Extensive numerical experiments showcasing the good long time behaviour of the scheme are summarised which are in agreement with the analysis proposed.

==> csv/dev/key.tex <==
%%% Explanation of deviation plots data

Figures show deviation in invariants from the initial value, thus
first value is exactly 0

scheme 9 and scheme 11 are both ldefocus (typo caused multiple names)
scheme 12 is defocus
ic 1 are the appropriate initial conditions from the paper
degree is the spatial polynomial degree

T = 100
dt = 1/1000
$x \in [0,40]$
dx = 0.25
